Dissection of a Bug Dataset: Anatomy of 395 Patches from Defects4J

Well-designed and publicly available datasets of bugs are an invaluable asset to advance research fields such as fault localization and program repair as they allow directly and fairly comparison between competing techniques and also the replication of experiments. These datasets need to be deeply understood by researchers: the answer for questions like "which bugs can my technique handle?" and "for which bugs is my technique effective?" depends on the comprehension of properties related to bugs and their patches. However, such properties are usually not included in the datasets, and there is still no widely adopted methodology for characterizing bugs and patches. In this work, we deeply study 395 patches of the Defects4J dataset. Quantitative properties (patch size and spreading) were automatically extracted, whereas qualitative ones (repair actions and patterns) were manually extracted using a thematic analysis-based approach. We found that 1) the median size of Defects4J patches is four lines, and almost 30% of the patches contain only addition of lines; 2) 92% of the patches change only one file, and 38% has no spreading at all; 3) the top-3 most applied repair actions are addition of method calls, conditionals, and assignments, occurring in 77% of the patches; and 4) nine repair patterns were found for 95% of the patches, where the most prevalent, appearing in 43% of the patches, is on conditional blocks. These results are useful for researchers to perform advanced analysis on their techniques' results based on Defects4J. Moreover, our set of properties can be used to characterize and compare different bug datasets.

==> pattern_example2save.tex <==
\captionsetup[subfigure]{font=small,skip=0pt,belowskip=5pt}
\begin{figure}
    \normalsize
%    \begin{minipage}[t]{\columnwidth}
    
    \begin{subfigure}[t]{\columnwidth}
    \begin{lstlisting} 
// Conditional Block Addition (Lang-45)
616 + if (lower > str.length()) {
617 +    lower = str.length();    
618 + }
// Conditional Block Addition with Return Statement (Closure-5)
176 + if (gramps.isDelProp()) {
177 +    return false;
178 + }
    \end{lstlisting}
    \caption*{Pattern 1 -- \textit{Conditional Block}.}
    \label{pattern:1}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Logic Expression Modification (Chart-1)
1797 - if (dataset != null) {
1797 + if (dataset == null) {
// Logic Expression Expansion (Mockito-34)
106 - if (m instanceof CapturesArguments) {            
106 + if (m instanceof CapturesArguments && i.getArguments().length > k) {
// Arithmetic Expression Modification (Math-69)
171 - out[i][j] = 2 * (1 - tDistribution.cumulativeProbability(t));            
171 + out[i][j] = 2 * tDistribution.cumulativeProbability(-t);
    \end{lstlisting}
    \caption*{Pattern 2 -- \textit{Expression Fix}.}
    \label{pattern:2}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Wraps-with if: Snippet showing 1 of 10 applications of the pattern (Time-3)
662 + if (years != 0) {
663    setMillis(getChronology().years().add(getMillis(), years));
664 + }
// Wraps-with if-else-exp (Mockito-29)
29 - description.appendText(wanted.toString());
29 + description.appendText(wanted == null ? "null" : wanted.toString());
// Unwraps-from method call computeFollowing(n) (Closure-85)
170 - Node fallThrough = tryRemoveUnconditionalBranching(computeFollowing(n));
170 + Node fallThrough = computeFollowing(n);
    \end{lstlisting}
    \caption*{Pattern 3 -- \textit{Wraps-with}.}
    \label{pattern:3}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Single Line Return Value Change (Math-5)
304   if (real == 0.0 && imaginary == 0.0) {
305 -    return NaN;            
305 +    return INF;            
306  }
    \end{lstlisting}
    \caption*{Pattern 4 -- \textit{Single Line}.}
    \label{pattern:4}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Wrong Variable Reference (Chart-11)
275 - PathIterator iterator2 = p1.getPathIterator(null);            
275 + PathIterator iterator2 = p2.getPathIterator(null);
// Wrong Method Reference (Closure-10)
1417 - return allResultsMatch(n, MAY_BE_STRING_PREDICATE);
1417 + return anyResultsMatch(n, MAY_BE_STRING_PREDICATE);
    \end{lstlisting}
    \caption*{Pattern 5 -- \textit{Wrong Reference}.}
    \label{pattern:5}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Missing Null-check and Not Null-check (Chart-15)
1378 +    if (this.dataset == null)  {
1379 +       return 0.0;
1380 +    }
    [...]
2054 +    if (this.dataset != null) {       
2055         state.setTotal(DatasetUtilities.calculatePieDatasetTotal(
2056                  plot.getDataset()));
2057 +    }
    \end{lstlisting}
    \caption*{Pattern 6 -- \textit{Missing Null-check}.}
    \label{pattern:6}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Copy/Paste of Method Call Replacement (Chart-4)
190 - if (detectImplicitPrototypeCycle()) {
190 + if (detectInheritanceCycle()) {
[...]
202 - if (detectImplicitPrototypeCycle()) {
202 + if (detectInheritanceCycle()) {
    \end{lstlisting}
    \caption*{Pattern 7 -- \textit{Copy/Paste}.}
    \label{pattern:7}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Change in the string literal (Closure 65)
1015 - case '\0': sb.append("\\0"); break;
1015 + case '\0': sb.append("\\000"); break;
// Replacement of a constant usage (Closure 75) 
375 - return TernaryValue.TRUE;
378 + return TernaryValue.UNKNOWN;
    \end{lstlisting}
    \caption*{Pattern 8 -- \textit{Constant Change}.}
    \label{pattern:8}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Move Code (Closure-13)
126 - traverse(c);            
126   Node next = c.getNext();            
127 + traverse(c);
    \end{lstlisting}
    \caption*{Pattern 9 -- \textit{Code Moving}.}
    \label{pattern:9}
    \vfill 
    \end{subfigure}
%    \end{minipage}
    \hfill
\caption{Code snippet examples for repair patterns.}
\label{fig:patterns}
\end{figure}

==> pattern_examples.tex <==
\captionsetup[subfigure]{font=small,skip=0pt,belowskip=5pt}
\begin{figure*}
    \normalsize
    \begin{minipage}[t]{\columnwidth}
    \begin{subfigure}[t]{\columnwidth}
    \begin{lstlisting} 
// Simple Conditional Block Addition
// Lang-45: org.apache.commons.lang.WordUtils
616 + if (lower > str.length()) {
617 +    lower = str.length();    
618 + }
// Conditional Block with Return Branch Addition
// Closure-5: com.google.javascript.jscomp.InlineObjectLiterals
176 + if (gramps.isDelProp()) {
177 +    return false;
178 + }
// Conditional Block with Exception Throwing Addition
// Math-48: org.apache.commons.math.analysis.solvers.BaseSecantSolver
189 + if (x == x1) {            
190 +    throw new ConvergenceException();            
191 + }
    \end{lstlisting}
    \caption*{\textbf{Pattern 1} - \textit{Conditional Block} (174 patches)}
    \label{pattern:1}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Wrap-With If 
// Snippet showing 1 of 10 applications of the pattern
// Time-3:  org.joda.time.MutableDateTime
662 + if (years != 0) {
663    setMillis(getChronology().years().add(getMillis(), years));
664 + } 
// Wraps-with If-Else
// Closure-56: com.google.javascript.jscomp.SourceFile
342 + if (pos >= js.length()) {
343      return null;
344 + } else {
345 +    return js.substring(pos, js.length());
346 + }
// Wraps-with If-Else-Exp
// Mockito-29: org.mockito.internal.matchers.Same
29 - description.appendText(wanted.toString());
29 + description.appendText(wanted == null ? "null" : wanted.toString());
// Unwrap Method Call computeFollowing(n)
// Closure-85: com.google.javascript.jscomp.UnreachableCodeElimination
170 - Node fallThrough = tryRemoveUnconditionalBranching(computeFollowing(n));
170 + Node fallThrough = computeFollowing(n);
// Unwrap If Conditional around rebuildIndex() call
// Chart-18: org.jfree.data.DefaultKeyedValues
318 - if (index < this.keys.size()) {
319      rebuildIndex();
320 - }
    \end{lstlisting}
    \caption*{\textbf{Pattern 3} - \textit{Wraps-with} (101 patches)}
    \label{pattern:3}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Missing Null-check and Not Null-check
// Chart-15: org.jfree.chart.plot.PiePlot
1377   public double getMaximumExplodePercent() {   
1378 +    if (this.dataset == null)  {
1379 +       return 0.0;
1380 +    }
1381      double result = 0.0; 
    [...]
2052      PiePlotState state = new PiePlotState(info);
2053      state.setPassesRequired(2);   
2054 +    if (this.dataset != null) {       
2055         state.setTotal(DatasetUtilities.calculatePieDatasetTotal(            
2056                  plot.getDataset()));            
2057 +    }
    \end{lstlisting}
    \caption*{\textbf{Pattern 5} - \textit{Missing Null-check} (59 patches)}
    \label{pattern:5}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Copy/Paste of Conditional Blocks with Null Check
// Chart-14: Adding 2 of 4 Null-Check in org.jfree.chart.plot.CategoryPlot and XYPlot
2155   public boolean removeDomainMarker(int index, Marker marker, Layer layer, boolean notify) {
       [...]
2166 + if (markers == null) {
2167 +    return false;
2168 + }
2169   boolean removed = markers.remove(marker);
       [...]
2437   public boolean removeRangeMarker(int index, Marker marker, Layer layer, boolean notify) {
       [...]
2451 + if (markers == null) {
2452 +    return false;
2453 + }
2454   boolean removed = markers.remove(marker);

    \end{lstlisting}
    \caption*{\textbf{Pattern 7} - \textit{Copy/Paste} (42 patches)}
    \label{pattern:7}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Move Code
// Closure-13: com.google.javascript.jscomp.PeepholeOptimizationsPass
126 - traverse(c);            
126   Node next = c.getNext();            
127 + traverse(c);
    \end{lstlisting}
    \caption*{\textbf{Pattern 9} - \textit{Code Moving} (6 patches)}
    \label{pattern:9}
    \vfill 
    \end{subfigure}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{\columnwidth}
    \begin{subfigure}[t]{\columnwidth}
    \begin{lstlisting} 
// Logic Expression Modifying
// Chart-1: org.jfree.chart.renderer.category.AbstractCategoryItemRenderer
1797 - if (dataset != null) {
1797 + if (dataset == null) {
// Logic Expression Expansion
// Closure-20: com.google.javascript.jscomp.PeepholeSubstituteAlternateSyntax
220 - if (value != null) { 
221 + if (value != null && value.getNext() == null && 
222 +      NodeUtil.isImmutableValue(value)) {
// Logic Expression Reduction
// Closure-18: com.google.javascript.jscomp.Compiler
1288 - if (options.dependencyOptions.needsManagement() && options.closurePass) {            
1288 + if (options.dependencyOptions.needsManagement()){
// Arithmetic Expression Modifying
// Math-69: org.apache.commons.math.stat.correlation.PearsonsCorrelation
171 - out[i][j] = 2 * (1 - tDistribution.cumulativeProbability(t));            
171 + out[i][j] = 2 * tDistribution.cumulativeProbability(-t);
    \end{lstlisting}
    \caption*{\textbf{Pattern 2} - \textit{Expression Fix} (137 patches)}
    \label{pattern:2}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Single Line Argument Value Change
// Chart-8: org.jfree.data.time.Week
175 - this(time, RegularTimePeriod.DEFAULT_TIME_ZONE, Locale.getDefault());            
175 + this(time, zone, Locale.getDefault());
// Single Line Return Value Change
// Math-5: org.apache.commons.math3.complex.Complex
304   if (real == 0.0 && imaginary == 0.0) {
305 -    return NaN;            
305 +    return INF;            
306  }
// Single Line Assignment Change
// Closure-71: com.google.javascript.jscomp.CheckAccessControls
416 - boolean isOverride = t.inGlobalScope() &&            
416 + boolean isOverride = parent.getJSDocInfo() != null &&
417        parent.getType() == Token.ASSIGN &&
418        parent.getFirstChild() == getprop;
// Single Line Method Replacement
// Math-75: org.apache.commons.math.stat.Frequency
303 - return getCumPct((Comparable<?>) v); 
303 + return getPct((Comparable<?>) v);

// Single Line Parameter Type Change
// Mockito-5: org.mockito.internal.verification.VerificationOverTimeImpl
91 - catch (org.mockito.exceptions.verification.junit.ArgumentsAreDifferent e) {            
91 + catch (AssertionError e) {
92      error = handleVerifyException(e);
    \end{lstlisting}
    \caption*{\textbf{Pattern 4} - \textit{Single Line} (85 patches)}
    \label{pattern:4}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Fix Initialization in Constructor Call
// Time-4: org.joda.time.Partial
464 - Partial newPartial = new Partial(iChronology, newTypes, newValues); 
464 + Partial newPartial = new Partial(newTypes, newValues, iChronology);
// Fix Initialization in Class Variable
// Math-104: org.apache.commons.math.special.Gamma
37 - private static final double DEFAULT_EPSILON = 10e-9;            
37 + private static final double DEFAULT_EPSILON = 10e-15;
// Fix Initialization of Local Variables
// Math-91: org.apache.commons.math.fraction.Fraction
259 - double nOd = doubleValue();            
259 + long nOd = ((long) numerator) * object.denominator;            
260 - double dOn = object.doubleValue();       
260 + long dOn = ((long) denominator) * object.numerator;
261   return (nOd < dOn) ? -1 : ((nOd > dOn) ? +1 : 0);
    \end{lstlisting}
    \caption*{\textbf{Pattern 6} - \textit{Initialization Fix} (44 patches)}
    \label{pattern:6}
    \vfill 
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
    \begin{lstlisting} 
// Wrong Reference to Object
// Chart-11: org.jfree.chart.util.ShapeUtilities
275 - PathIterator iterator2 = p1.getPathIterator(null);            
275 + PathIterator iterator2 = p2.getPathIterator(null);
// Wrong Reference in Argument of Method Call
// Lang-6: org.apache.commons.lang3.text.translate.CharSequenceTranslator
95 - pos += Character.charCount(Character.codePointAt(input, pos));            
95 + pos += Character.charCount(Character.codePointAt(input, pt));
// Wrong Reference - Direct Object Access to Method Call
// Lang-57: org.apache.commons.lang.LocaleUtils
223 - return cAvailableLocaleSet.contains(locale);    
223 + return availableLocaleList().contains(locale);
    \end{lstlisting}
    \caption*{\textbf{Pattern 8} - \textit{Wrong reference} (21 patches)}
    \label{pattern:8}
    \vfill 
    \end{subfigure}
    \end{minipage}
\caption{Repair Patterns code examples.}
\label{fig:patterns}
\end{figure*}
